ADOP: Approximate Differentiable One-Pixel Point Rendering

In this paper we present ADOP, a novel point-based, differentiable neural rendering pipeline. Like other neural renderers, our system takes as input calibrated camera images and a proxy geometry of the scene, in our case a point cloud. To generate a novel view, the point cloud is rasterized with learned feature vectors as colors and a deep neural network fills the remaining holes and shades each output pixel. The rasterizer renders points as one-pixel splats, which makes it very fast and allows us to compute gradients with respect to all relevant input parameters efficiently. Furthermore, our pipeline contains a fully differentiable physically-based photometric camera model, including exposure, white balance, and a camera response function. Following the idea of inverse rendering, we use our renderer to refine its input in order to reduce inconsistencies and optimize the quality of its output. In particular, we can optimize structural parameters like the camera pose, lens distortions, point positions and features, and a neural environment map, but also photometric parameters like camera response function, vignetting, and per-image exposure and white balance. Because our pipeline includes photometric parameters, e.g.~exposure and camera response function, our system can smoothly handle input images with varying exposure and white balance, and generates high-dynamic range output. We show that due to the improved input, we can achieve high render quality, also for difficult input, e.g. with imperfect camera calibrations, inaccurate proxy geometry, or varying exposure. As a result, a simpler and thus faster deep neural network is sufficient for reconstruction. In combination with the fast point rasterization, ADOP achieves real-time rendering rates even for models with well over 100M points. https://github.com/darglein/ADOP

==> common/5_Discard.tex <==
\section{Adaptive Point Discarding}
\label{sec:architecture}
The most common data structure for real-time 3d reconstruction from depth images is a truncated signed distance field (TSDF).
Each voxel stores the signed distance to the surface up to a threshold $t_d$.
Voxels with a distance larger than $t_d$ are not relevant and can be discarded.
It has been shown, that a sparse structure of voxel blocks can reduce memory consumption significantly and allows real-time operation on large-scale scenes.
This structure consist of $N$ blocks of $d^3$ voxels, in our case $d=8$, with $C$ channels each and is stored using a data tensor D and a structure tensor S.


==> common/6_Ablation.tex <==
%\subsection{Ablation Studies}



%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX
%% NOT USED ANYMORE, COPY PASTED IN EXPERIMENTS.TEX



\paragraph{Loss Function} 
%Several loss functions have been used for training in previous work, in particular mean squared error (MSE) \cite{mildenhall2020nerf,zhang2020nerfpp} and the VGG perceptual loss \cite{johnson2016perceptual}, used by \cite{aliev2020neural}.

We have trained ADOP on the M60 scene using typical loss function also used in prior work: L1 and MSE, the VGG perceptual loss \cite{johnson2016perceptual}, the LPIPS loss \cite{zhang2018perceptual}, the peak signal-to-noise ratio (PSNR), and the structured similarity index (SSIM).
The results are shown in Fig.~\ref{fig:abl_loss}.
Using the VGG loss, the most details are visible and the overall sharpness is significantly improved compared to the other losses.
All further experiments are therefore conducted using VGG as the loss function.

\begin{figure}
	\centering
		\includegraphics[width=\linewidth]{out/ablation_loss.pdf}
	\vspace{0.05cm}
	\ifx\arxivsubmission\undefined
	\small
	\fi

	\centering
\begin{tabular}{@{}l|lll|lll@{}}
\toprule
               & L1 $\downarrow$            & MSE   $\downarrow$          & VGG   $\downarrow$          & PSNR   $\uparrow$        & LPIPS $\downarrow$         & SSIM  $\uparrow$         \\ \midrule
Train w. L1  & \textbf{0.029} & \textbf{0.0033} & 487.43          & \textbf{25.10} & 0.264          & \textbf{0.846} \\
Train w. MSE & 0.034          & 0.0037          & 558.84          & 24.67          & 0.322          & 0.822          \\
Train w. VGG & 0.032          & 0.0035          & \textbf{357.08} & 24.79          & \textbf{0.145} & 0.804          \\ \bottomrule
\end{tabular}
	\captionof{figure}{
		Effect of training ADOP with different loss functions.
		Using the VGG loss for training improves the image quality significantly even though some metrics favor a training with L1 loss.
	}
	\label{fig:abl_loss}
	
\end{figure}



\paragraph{Ablation Study}

\begin{figure}
	\centering
		\includegraphics[width=\linewidth]{out/ablation_modules.pdf}
	\vspace{0.05cm}
	\ifx\arxivsubmission\undefined
	\small
	\fi

	\centering
\begin{tabular}{@{}l|lll|lll@{}}
\toprule
                          & \multicolumn{3}{c|}{Playground}                   & \multicolumn{3}{c}{Train}                         \\
                          & VGG            & LPIPS           & Diff           & VGG            & LPIPS           & Diff           \\ \midrule
Baseline                  & 374.8          & 0.1761          &               & 514.3          & 0.2116          &               \\
\ \ + Env.                    & 374.8          & 0.1734          & -1.5\%         & 490.8          & 0.1937          & -8.5\%         \\
\ \ + Env. + TM               & 352.2          & 0.1655          & -6.0\%         & 412.0          & 0.1614          & -24\%          \\
\ \ \textbf{+ Env. + TM + SO} & \textbf{318.7} & \textbf{0.1464} & \textbf{-17\%} & \textbf{358.1} & \textbf{0.1438} & \textbf{-32\%} \\ \bottomrule
\end{tabular}
	\captionof{figure}{
		Ablation study on the major contributions of ADOP.
		Enabling the enviroment map (Env), the tone mapper (TM), and the structure optimization (SO) noticeable improves the sharpness and color accuracy.
	}
	\label{fig:abl_modules}
	
\end{figure}

Compared to previous work of neural point-based rendering, we have proposed several ideas to improve the quality of novel view synthesis.
In Figure \ref{fig:abl_modules}, we analyze how much each module contributes to the final result.
The first row shows a baseline experiment, which is similar to NPBG \cite{aliev2020neural}.
After that we enable one by one, the environment map (Env), the tone mapper (TM), and the structure optimization (SO).
In the latter, we initialize the scene using the COLMAP reconstruction and then optimize the camera pose, camera model, and point cloud during the training stage.
All together, a significant improvement in image quality is achieved with a LPIPS loss reduction of 17\% on the playground scene and 32\% on the train scene.

\paragraph{Robust Pose Correction}
\begin{figure}
	\centering
		\includegraphics[width=\linewidth]{out/ablation_pose.pdf}
		
		\vspace{0.1cm}
		
			\begin{tikzpicture}
				\begin{axis}[
					height=5cm,
					width=0.8\linewidth,
					at={(0,0)},
					ymin=250,
					ymax=700,
					xmin=0,
					xmax=400,
					%grid=both,
					minor tick num =1,
					minor tick style={draw=none},
					%minor grid style={thin,color=black!10},
					%major grid style={thin,color=black!10},
					ylabel=VGG (Train),
					xlabel=Epoch,
					%  tick align=outside,
					legend style={font=\small},
					xlabel style={font=\small},
					ylabel style={font=\small},
					x tick label style={
						/pgf/number format/assume math mode, font=\tiny},
					y tick label style={
						/pgf/number format/assume math mode, font=\tiny},
					]
					\addplot[color=red,tension=0.7] table [x=ep, y=vgg, col sep=comma] {../../images/ablation_pose/ref_loss.txt};
					\addplot[color=blue,tension=0.7] table [x=ep, y=vgg, col sep=comma] {../../images/ablation_pose/no_op_loss.txt};
					\addplot[color=green,tension=0.7] table [x=ep, y=vgg, col sep=comma] {../../images/ablation_pose/op_loss.txt};
					
					\legend{COLMAP, COLMAP + Noise, COLMAP + Noise + SO}	

				\end{axis}
			\end{tikzpicture}
			
			\caption{
			Without structure optimization (SO), neural point-based rendering is sensitive to a bad initialization resulting in severe image artifacts (top right).
			However, our SO technique can recover from the erroneous input and can even outperform the COLMAP initialization after 400 training epochs (bottom left).
			}
			\label{fig:abl_pose}
\end{figure}
In the previous study, we have shown that structure optimization improves rendering quality when using the initial COLMAP reconstruction.
To further prove the robustness of our approximate gradient computation (see Section \ref{sec:backward}), we now add Gaussian noise to the camera position and rotation.
As shown in Figure~\ref{fig:abl_pose}, the result is practically identical to not adding pose noise.
ADOP is therefore robust to a bad initial calibration and can also be used for image to point cloud alignment (see Appendix~\ref{sec:image2points}).
Without pose optimization (right column) strong blur and ghosting artifacts are visible due to the misaligned frames.

\paragraph{Unet Layers}
\begin{figure}
	\centering
		\includegraphics[width=\linewidth]{out/ablation_layers.pdf}
	\vspace{0.05cm}
	\ifx\arxivsubmission\undefined
	\small
	\fi

	\centering
\begin{tabular}{@{}l|r|c|ll|ll@{}}
         & \multicolumn{1}{l|}{}         & Train Loss     & \multicolumn{2}{c|}{Test Loss}   & \multicolumn{2}{c}{Time (ms)} \\
         & \multicolumn{1}{l|}{\#Params} & VGG            & VGG            & LPIPS           & FP32             & FP16            \\ \midrule
3 Layers & 136387                        & 302.5          & 330.9          & 0.1364          & \textbf{34.264}  & \textbf{22.604} \\
4 Layers & 574651                        & 262.8          & \textbf{317.0} & \textbf{0.1191} & 41.343           & 26.665          \\
5 Layers & 2335923                       & \textbf{245.7} & 325.8          & 0.1239          & 48.106           & 30.798          \\ \bottomrule
\end{tabular}
	\captionof{figure}{
		Quality comparison on the number of Unet-layers inside the neural renderer.
		More layers improves the hole-filling capabilities (see images) but also reduces rendering efficiency.
		On some scenes, a 5 layer network is also prone to overfit on the training images (low train loss, but high test loss).
	}
	\label{fig:abl_layers}
\end{figure}
In Section \ref{sec:pipeline}, we have mentioned that we use a 4-Layer Unet as neural renderer.
Since other methods often use a 5-Layer network instead \cite{aliev2020neural,thies2019deferred}, we show in Figure \ref{fig:abl_layers} the difference between these approaches.
The rendering quality is almost identical on all of our scenes. 
However, a 4-Layer network has slightly improved efficiency and is less prone to overfitting the training images.
We therefore set the default to 4 layers but recommend the user to test both options on new scenes.
A five layer network has improved hole-filling capabilities and therefore might be preferred on scenes with sparse point clouds.




\paragraph{Stochastic Point Discarding}

\begin{figure}
	\centering
		\includegraphics[width=\linewidth]{out/ablation_discarding.pdf}
	\captionof{figure}{
		Stochastic discarding roughly halfes the number of blended points, which increaes rasterization efficiency by 15-25\%.
		The image quality is visually and quantitatively not affected.
	}
	\label{fig:abl_disc}
	
\end{figure}

\begin{figure}
	\centering
		\includegraphics[width=\linewidth]{out/extreme_view.pdf}
	\captionof{figure}{
		View extrapolation with a large distance to the closest training image.
		Our method can retain a reasonable sharp image from arbitrary camera locations.
		\LF{Do you want a nerf++ image as well?}
		\LF{Also, SVS is not really introduced at this point, cite or later?}
	}
	\label{fig:extrapolation}
	
\end{figure}


In Section \ref{sec:point_discarding} we have proposed a stochastic point discarding technique to reduce the pixel-overdraw without impacting rendering quality.
To verify this assumption we train ADOP with and without point discarding on the Kemenate and Lighthouse dataset.
\LF{Only the kemenate scene is shown, maybe add lighthouse to appendix?}
We measure the number of blending operations, render time, and image quality.
The result is present in Figure \ref{fig:abl_disc}.
Visually we cannot spot a difference between these two configurations, which is backed by the perceptual rendering loss.
However, in average only 50\% of the points are blended, which reduces rendering time by 20\%.


